Achievable Information Rates and Concatenated Codes for the DNA Nanopore Sequencing Channel

The errors occurring in DNA-based storage are correlated in nature, which is a direct consequence of the synthesis and sequencing processes. In this paper, we consider the memory-$k$ nanopore channel model recently introduced by Hamoum et al., which models the inherent memory of the channel. We derive the maximum a posteriori (MAP) decoder for this channel model. The derived MAP decoder allows us to compute achievable information rates for the true DNA storage channel assuming a mismatched decoder matched to the memory-$k$ nanopore channel model, and quantify the loss in performance assuming a small memory length--and hence limited decoding complexity. Furthermore, the derived MAP decoder can be used to design error-correcting codes tailored to the DNA storage channel. We show that a concatenated coding scheme with an outer low-density parity-check code and an inner convolutional code yields excellent performance.

==> Figures/AIRs_dataset_vs_model.tex <==
 \begin{figure}[t!]
 \centering \centering

\begin{comment}
    

	\begin{tikzpicture}
		\begin{axis}[
			width = 1\columnwidth,
			%height = 7.43cm
			xmin=1,   xmax=10,
			ymin=0.8,	ymax=1.6,
			%xticklabel={\ifdim\tick pt=0pt 0 \else\pgfmathprintnumber{\tick}\fi},
			xtick distance = 1,
			xticklabel style = {/pgf/number format/fixed, /pgf/number format/precision=2},
			grid = both,
			grid style = {line width=.1pt},
			%legend columns=2,
            legend cell align=left,
            legend style={at={(axis cs: 9.8,0.82)},anchor=south east},
			legend style={font=\tiny},
			xlabel = {$\numS$},
			ylabel style = {name=AIR,yshift=-.0cm},
			ylabel = {$R_{\text{BCJR-once}}$},
			]
			
			
\addplot [line width=0.75pt,mark=x, color=black, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_iidDecoding_Uncoded_k1_N110_Orate_LLR.txt};
\addlegendentry{\tiny i.i.d. decoding};

\addplot [line width=0.75pt,mark=square*, color=blue, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k1_N110_Orate_LLR.txt};
\addlegendentry{\tiny $k = 1$};

\addplot [line width=0.75pt,mark=pentagon*, color=violet, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k2_N110_Orate_LLR.txt};
\addlegendentry{\tiny $k = 2$};

\addplot [line width=0.75pt,mark=diamond*, color=red, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k3_N110_Orate_LLR.txt};
\addlegendentry{\tiny $k = 3$};

\addplot [line width=0.75pt,mark=*, color=ColorIGMDDSR, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k5_N110_Orate_LLR.txt};
\addlegendentry{\tiny $k = 5$};

\addplot [line width=0.75pt,mark=x, color=cyan, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k6_N110_Orate_LLR.txt};
\addlegendentry{\tiny $k = 6$};

\addplot [line width=0.75pt,mark=triangle*, color=orange, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k7_N110_Orate_LLR.txt};
\addlegendentry{\tiny $k = 7$};



\addplot [line width=0.75pt,mark=square*, color=blue, dashed, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k1_N110_Orate_LLR_2.txt};

\addplot [line width=0.75pt,mark=pentagon*, color=violet, dashed, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k2_N110_Orate_LLR_2.txt};

\addplot [line width=0.75pt,mark=diamond*, color=red, dashed, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k3_N110_Orate_LLR_2.txt};


\addplot [line width=0.75pt,mark=*, color=ColorIGMDDSR, dashed, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k5_N110_Orate_LLR_2.txt};

\addplot [dashed, line width=0.75pt,mark=x, color=cyan, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k6_N110_Orate_LLR_2.txt};
%\addlegendentry{\tiny $k = 6$};
			
\addplot [line width=0.75pt,mark=triangle*, color=orange, dashed, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_Uncoded_k7_N110_Orate_LLR_2.txt};



%\addplot [dashed, line width=0.75pt,mark=square*, color=blue, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_CC_k1_N112_Orate_LLR.txt};
%\addlegendentry{\tiny $k = 1$};
%\addplot [dashed, line width=0.75pt,mark=pentagon*, color=violet, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_CC_k2_N112_Orate_LLR.txt};
%\addlegendentry{\tiny $k = 2$};

%\addplot [dashed, line width=0.75pt,mark=square*, color=blue, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_CC_0.75_k1_N112_Orate_LLR.txt};

%\addplot [dashed, line width=0.75pt,mark=pentagon*, color=violet, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_CC_0.75_k2_N112_Orate_LLR.txt};


%\addplot [dashed, line width=0.75pt,mark=*, color=ColorIGMDDSR, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=AIR] {Figures/AIR_DNA_corrolatedChannel_CC_0.75_k5_N112_Orate_LLR.txt};

%\draw[black, dashed] (axis cs: 3,1.30) ellipse (0.3cm and 1.0cm) node at (axis cs: 3,1.15) {\footnotesize Uncoded};

%\draw[black, dashed] (axis cs: 3,0.99) ellipse (0.3cm and 0.5cm) node at (axis cs: 3,0.89) {\footnotesize CC-1};

%\draw[black, dashed] (axis cs: 1.5,1.32) ellipse (0.2cm and 0.5cm) node at (axis cs: 1.5,1.4) {\footnotesize CC-2};	

		\end{axis}
	\end{tikzpicture}
 \end{comment}
 \includegraphics[scale = 0.7]{Figures/AIRs_dataset_vs_model_pic.pdf}
	\vspace{-5ex}
	\caption{BCJR-once rates with no inner code for different values of $M$ and $N=110$. Solid curves are for the true channel and dashed curves are for a memory-$k$ nanopore channel model.}
	\label{fig:BCJR-Once-Inner_DS_vs_Model}
	\vspace{-4ex}
	 \end{figure}

==> Figures/FER_plots.tex <==
%\begin{figure}[t!]

%\centering \centering

%\resizebox{0.8\paperwidth}{!}{%
%\begin{tikzpicture}%[thick, scale=0.9, every node/.style={transform shape}]
%\pgfplotsset{every tick label/.append style={font=\small}}
%\begin{axis}[%


\addplot [line width=0.75pt, mark=*, color=ColorIGMDDSR, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=FER] {Figures/Conc_code_DNA_kmer-len5_corrChannel_CC(2,1,2)+LDPC(2,10)_Optimized_n10000_k8000_dataset.txt};
%\addlegendentry{$k = 5$};


\addplot [dashed, line width=0.75pt, mark=*, color=ColorIGMDDSR, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=FER] {Figures/Conc_code_DNA_kmer-len5_corrChannel_CC(2,1,2)+LDPC(2,10)_Optimized_n10000_k8000.txt};


\addplot [dashdotted, line width=0.75pt, mark=diamond*, color=red, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=FER] {Figures/Conc_code_DNA_kmer-len5Channel_kmer-len3Decoding_corrChannel_CC(2,1,2)+LDPC(2,10)_Optimized_n10000_k8000.txt};

%\addlegendentry{$k = 5$};

%\addplot [line width=0.75pt, mark=*, color=red, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=FER] {Figures/Conc_code_DNA_kmer-len5_corrChannel_CC(2,1,2)+LDPC(3,6)_Optimized_n228_k114_R05.txt};
%\addlegendentry{$k$ = 5, $R_o = 4/8$.};

%\addplot [line width=0.75pt, mark=triangle*, color=orange, mark options={solid, fill=white}] table [col sep=space, x=numSeq, y=FER] {Figures/Conc_code_DNA_kmer-len5_corrChannel_CC(2,1,2)+LDPC(3,6)_Optimized_n228_k114_R0375.txt};
%\addlegendentry{$k$ = 5, $R_o = 3/8$.};

%\end{axis}
%\end{tikzpicture}%
%\vspace{-3ex}
	%\caption{FER performance of the  optimized concatenated  codes versus the number of received sequences $M$ decoded using separate decoding  for $N=110$ and with different levels of decoder mismatch. %The binary outer LDPC codes are of length $\leno=10000$ and were constructed from the protographs in Table~\ref{tab:DE_protographs}.
	%The solid curves are for the true channel, while the dashed curves are for a memory-$5$  channel model.} %The overall code rate is $R = \rateo \ratei = \nicefrac{8}{10} \cdot \nicefrac{3}{2}=\nicefrac{6}{5}$.}
	%\label{fig:FER}
	%\vspace{-3ex}
%\end{figure}

